OpenWorldLib: A Unified Codebase and Definition of Advanced World Models

World models have garnered significant attention as a promising research direction in artificial intelligence, yet a clear and unified definition remains lacking. In this paper, we introduce OpenWorldLib, a comprehensive and standardized inference framework for Advanced World Models. Drawing on the evolution of world models, we propose a clear definition: a world model is a model or framework centered on perception, equipped with interaction and long-term memory capabilities, for understanding and predicting the complex world. We further systematically categorize the essential capabilities of world models. Based on this definition, OpenWorldLib integrates models across different tasks within a unified framework, enabling efficient reuse and collaborative inference. Finally, we present additional reflections and analyses on potential future directions for world model research. Code link: https://github.com/OpenDCAI/OpenWorldLib

==> tables/agenticrag.tex <==
\begin{table}
\centering
\small
\caption{AgenticRAG Pipeline: Performance comparison between synthetic datasets and existing human-constructed datasets. All values are Exact Match (\%). ``OOD-Avg'' excludes the in-domain test set of each training dataset. ``DF-OOD (matched)'' provides the OOD score of DF-AgenticRAG under the *same* in-domain exclusion, ensuring fair comparison.}
\label{tab:agenticrag}
\resizebox{\textwidth}{!}{
\begin{tabular}{lccccccc}
\toprule
\textbf{Training Data} & \textbf{HotpotQA} & \textbf{2Wiki} & \textbf{Musique} & \textbf{Bamboogle} & \textbf{Avg} & \textbf{OOD-Avg} & \textbf{DF-OOD (matched)} \\
\midrule
Qwen-2.5-7B-Instruct & 25.0 & 25.8 & 9.9 & 27.2 & 22.0 & -- & -- \\
\midrule

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%               HotpotQA group
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\rowcolor[rgb]{.867,.922,.969}
\multicolumn{8}{c}{\textit{\textbf{Trained on HotpotQA (in-domain = HotpotQA)}}} \\
\midrule

HotpotQA-10k (1 epoch) & 40.2 & 41.9 & 16.7 & 42.4 & 35.3 & 33.7 & \textbf{33.8} \\
HotpotQA-10k (2 epochs) & 43.4 & 44.9 & 18.9 & 41.6 & 37.2 & 35.1 & \textbf{35.9} \\
HotpotQA-10k (3 epochs) & 45.3 & 48.0 & 20.3 & 40.8 & 38.6 & 36.4 & \textbf{37.4} \\

\midrule

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%               Musique group
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\rowcolor[rgb]{.867,.922,.969}
\multicolumn{8}{c}{\textit{\textbf{Trained on Musique (in-domain = Musique)}}} \\
\midrule

Musique-20k (1 epoch) & 41.1 & 44.7 & 19.2 & 41.6 & 36.6 & 42.4 & \textbf{43.6} \\

\midrule

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%               2Wiki group
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\rowcolor[rgb]{.867,.922,.969}
\multicolumn{8}{c}{\textit{\textbf{Trained on 2Wiki (in-domain = 2Wiki)}}} \\
\midrule

2Wiki-30k (2 epochs) & 41.3 & 55.1 & 17.8 & 42.4 & 39.1 & 33.8 & \textbf{36.4} \\

\midrule

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%            DF-AgenticRAG raw
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\rowcolor[rgb]{.867,.922,.969}
\multicolumn{8}{c}{\textit{\textbf{DF-AgenticRAG (raw results, for reference)}}} \\
\midrule

DataFlow-AgenticRAG-10k (1 epoch) & 39.3 & 42.6 & 17.3 & 41.6 & 34.3 & -- & -- \\
DataFlow-AgenticRAG-10k (2 epochs) & 43.1 & 44.6 & 19.9 & 43.2 & 37.7 & -- & -- \\
DataFlow-AgenticRAG-10k (3 epochs) & 42.6 & 45.5 & 20.2 & 46.4 & 38.7 & -- & -- \\

\bottomrule
\end{tabular}
}
\end{table}


==> tables/code_1.tex <==
\begin{table}[t]
\centering
\small
\caption{Performance comparison of Qwen2.5-7B and Qwen2.5-14B under different SFT dataset settings (all numbers in \%).}
\label{tab:code_1}
\resizebox{\textwidth}{!}{
\begin{tabular}{lccccc}
\toprule
\textbf{Model} & \textbf{HumanEval} & \textbf{MBPP} & \textbf{BigCodeBench} & \textbf{LiveCodeBench} & \textbf{Avg} \\
\midrule
\rowcolor[rgb]{.867, .922, .969}
\multicolumn{6}{c}{\textit{\textbf{Trained on Qwen2.5-7B}}} \\
\midrule
Original & 57.9 & 74.9 & 37.5 & 2.5  & 43.2 \\
Code Alpaca & 76.2 & 76.5 & 43.8 & 6.0  & 50.6 \\
Self-OSS-Instruct-SC2-Exec-Filter-50k & 74.4 & 77.0 & 42.7 & 6.1  & 50.1 \\
DataFlow-Code-1K & 75.0 & 75.4 & 46.2 & 21.5 & 54.5 \\
DataFlow-Code-5K & 78.7 & 77.2 & 46.1 & 22.1 & 56.0 \\
DataFlow-Code-10K & 78.7 & 78.3 & 45.9 & 23.0 & \textbf{56.5} \\
\midrule
\rowcolor[rgb]{.867, .922, .969}
\multicolumn{6}{c}{\textit{\textbf{Trained on Qwen2.5-14B}}} \\
\midrule
Original & 56.7 & 76.7 & 53.4 & 21.2 & 52.0 \\
Code Alpaca & 81.5 & 78.8 & 53.3 & 21.9 & 58.9 \\
Self-OSS-Instruct-SC2-Exec-Filter-50k & 82.0 & 81.0 & 52.2 & 23.6 & 59.7 \\
DataFlow-Code-1K & 77.6 & 82.5 & 53.9 & 27.6 & 60.4 \\
DataFlow-Code-5K & 79.9 & 84.1 & 54.2 & 27.8 & 61.5 \\
DataFlow-Code-10K & 81.1 & 84.5 & 54.1 & 30.0 & \textbf{62.4} \\
\bottomrule
\end{tabular}
}
\end{table}



==> tables/code_2.tex <==
\begin{table}[t]
\centering
\small
\caption{Code Pipeline: Performance comparison of Qwen2.5-7B-Instruct and Qwen2.5-14B-Instruct under different SFT dataset settings (all numbers in \%).}
\label{tab:code_2}
\resizebox{\textwidth}{!}{
\begin{tabular}{lcccccc}
\toprule
\textbf{Training Data} & \textbf{BigCodeBench} & \textbf{LiveCodeBench(v6)} & \textbf{CruxEval (Input)} & \textbf{CruxEval (Output)} & \textbf{HumanEval+} & \textbf{Avg} \\
\midrule

\rowcolor[rgb]{.867, .922, .969}
\multicolumn{7}{c}{\textit{\textbf{Trained on Qwen2.5-7B-Instruct}}} \\
\midrule
\textbf{Qwen2.5-7B-Instruct}              & 35.3 & 23.4 & 44.8 & 43.9 & 72.6 & 44.0 \\
\textbf{+ Code Alpaca-1K}        & 33.3 & 18.7 & 45.6 & 46.4 & 66.5 & 42.1 \\
\textbf{+ Self-OSS}              & 31.9 & 21.4 & 46.9 & 45.9 & 70.1 & 43.2 \\
\textbf{+ DataFlow-Code-1K}      & 35.5 & 25.7 & 48.0 & 45.1 & 72.6 & 45.4 \\
\textbf{+ DataFlow-Code-5K}      & 36.2 & \textbf{26.4} & 48.6 & 45.0 & 73.2 & 45.9 \\
\textbf{+ DataFlow-Code-10K}     & \textbf{36.8} & 26.0 & \textbf{48.8} & \textbf{45.4} & \textbf{73.8} & \textbf{46.2} \\
\midrule
\rowcolor[rgb]{.867, .922, .969}
\multicolumn{7}{c}{\textit{\textbf{Trained on Qwen2.5-14B-Instruct}}} \\
\midrule
\textbf{Qwen2.5-14B-Instruct}              & 37.5 & 33.4 & 48.0 & 48.5 & 74.4 & 48.4 \\
\textbf{+ Code Alpaca-1K}        & 37.0 & 28.2 & 50.2 & 49.6 & 71.3 & 47.3 \\
\textbf{+ Self-OSS}              & 36.9 & 22.3 & 52.6 & 50.1 & 68.3 & 46.0 \\
\textbf{+ DataFlow-Code-1K}      & 41.4 & \textbf{33.7} & 51.0 & 50.9 & \textbf{77.3} & 50.9 \\
\textbf{+ DataFlow-Code-5K}      & 41.1 & 33.2 & 52.5 & 50.6 & 76.2 & 50.7 \\
\textbf{+ DataFlow-Code-10K}     & \textbf{41.9} & 33.2 & \textbf{52.9} & \textbf{51.0} & 76.2 & \textbf{51.0} \\
\bottomrule
\end{tabular}
}
\end{table}


==> tables/dfa_table1.tex <==
\begin{table*}[!h]
\centering
\caption{Agent orchestration performance by evaluation mode and description difficulty.}
\label{tab:agent-orchestration-results-vertical}

\setlength{\tabcolsep}{6pt}
\renewcommand{\arraystretch}{1.15}
\small

\begin{tabular}{lcccc}
\toprule
\textbf{Metric} & \textbf{Easy} & \textbf{Medium} & \textbf{Hard} & \textbf{Overall} \\
\midrule

\multicolumn{5}{l}{\textbf{Text spec evaluation (pipeline mode)}}\\
\midrule
Avg. LLM-Judge & 0.92 & 0.86 & 0.60 & 0.80 \\
\midrule

\multicolumn{5}{l}{\textbf{Code GT evaluation (code mode)}}\\
\midrule
Avg. LLM-Judge & 0.60 & 0.59 & 0.23 & 0.49 \\
\bottomrule
\end{tabular}
\end{table*}

==> tables/general_1.tex <==
\begin{table}[t]
\centering
\small
\caption{Performance of \textsc{DataFlow-Instruct-10K} on Math Benchmarks: Qwen2-7B-Base and Qwen2.5-7B-Base finetuned series of models (Exact Match \%). }
%Blue numbers highlight DF-Gen-10K finetuning, and red numbers highlight the corresponding Instruct checkpoints.
\label{tab:general_math}
\resizebox{\textwidth}{!}{
\begin{tabular}{lcccccccc}
\toprule
\textbf{Model} 
& \textbf{MATH} & \textbf{GSM8K} & \textbf{AMC23} & \textbf{AIME24} 
& \textbf{Minerva} & \textbf{Gaokao} & \textbf{Olympiad} & \textbf{Math-Avg} \\
\midrule
\rowcolor[rgb]{.867, .922, .969}
\multicolumn{9}{c}{\textit{\textbf{Models based on Qwen2-7B}}} \\
\midrule
\textbf{Qwen2-7B-Base}                             & 21.2 & 55.9 & 15.0 & 0.0 &  9.9 & 30.8 &  7.7 & 20.1 \\
\textbf{\quad + Inf-10K}                           & 45.6 & 81.7 & 25.0 & 3.3 & 11.8 & 24.2 & 11.1 & 29.0 \\
\textbf{\quad + Inf-1M}                            & 45.4 & 79.2 & 25.0 & 0.0 & 13.2 & 22.0 & 10.4 & 27.9 \\
\textbf{\quad + \textsc{DataFlow-Instruct-10K}}                        & 54.0 & 83.0 & 27.5 & 0.0 & 16.5 & 25.3 & 20.3 & \textcolor{blue}{32.4} \\
\textbf{Qwen2-7B-Instruct}                         & 53.9 & 86.2 & 22.5 & 3.3 & 17.6 & 35.2 & 19.6 & \textcolor{red}{34.0} \\
\midrule
\rowcolor[rgb]{.867, .922, .969}
\multicolumn{9}{c}{\textit{\textbf{Models based on Qwen2.5-7B}}} \\
\midrule
\textbf{Qwen2.5-7B-Base}                           & 62.8 & 67.1 & 45.0 & 10.0 & 17.6 & 27.5 & 29.6 & 37.1 \\
\textbf{\quad + Inf-10K}                           & 40.2 & 30.9 & 25.0 & 3.3  &  9.2 & 27.5 & 21.8 & 22.6 \\
\textbf{\quad + Inf-1M}                            & 50.6 & 82.0 & 27.5 & 0.0  & 22.1 & 30.8 & 20.0 & 33.3 \\
\textbf{\quad + \textsc{DataFlow-Instruct-10K}}                        & 73.8 & 88.2 & 47.5 & 16.7 & 30.9 & 31.9 & 37.6 & \textcolor{blue}{46.7} \\
\textbf{Qwen2.5-7B-Instruct}                       & 75.1 & 92.4 & 47.5 & 10.0 & 34.9 & 48.4 & 40.6 & \textcolor{red}{49.8} \\
\bottomrule
\end{tabular}
}
\end{table}


==> tables/general_2.tex <==
\begin{table}[t]
\centering
\small
\caption{Performance of \textsc{DataFlow-Instruct-10K} on Code and Knowledge benchmarks: Qwen2-7B-Base and Qwen2.5-7B-Base finetuned models.}
\label{tab:general_code_knowledge}
\resizebox{\textwidth}{!}{
\begin{tabular}{lcccccc}
\toprule
\textbf{Model} 
& \textbf{HumanEval} & \textbf{MBPP} & \textbf{Code-Avg} 
& \textbf{MMLU} & \textbf{C-EVAL} & \textbf{Knowledge-Avg} \\
\midrule
\rowcolor[rgb]{.867, .922, .969}
\multicolumn{7}{c}{\textit{\textbf{Models based on Qwen2-7B}}} \\
\midrule
\textbf{Qwen2-7B-Base}                      & 66.5 & 66.1 & 66.3                 & 69.6 & 82.8 & \textcolor{red}{76.2} \\
\textbf{\quad + Inf-10K}                    & 64.0 & 71.7 & 67.8                 & 69.3 & 83.0 & \textcolor{red}{76.2} \\
\textbf{\quad + Inf-1M}                     & 65.9 & 70.4 & \textcolor{blue}{68.2} & 69.5 & 83.0 & \textcolor{red}{76.2} \\
\textbf{\quad + \textsc{DataFlow-Instruct-10K}}                 & 64.6 & 67.7 & 66.2                 & 69.4 & 82.8 & \textcolor{blue}{76.1} \\
\textbf{Qwen2-7B-Instruct}                  & 73.8 & 65.3 & \textcolor{red}{69.6}  & 69.9 & 82.0 & 76.0 \\
\midrule
\rowcolor[rgb]{.867, .922, .969}
\multicolumn{7}{c}{\textit{\textbf{Models based on Qwen2.5-7B}}} \\
\midrule
\textbf{Qwen2.5-7B-Base}                    & 78.7 & 74.3 & 76.5                 & 71.9 & 80.0 & \textcolor{blue}{76.0} \\
\textbf{\quad + Inf-10K}                    & 77.4 & 77.8 & 77.6                 & 71.8 & 79.9 & 75.8 \\
\textbf{\quad + Inf-1M}                     & 78.0 & 78.0 & 78.0                 & 72.2 & 79.4 & 75.8 \\
\textbf{\quad + \textsc{DataFlow-Instruct-10K}}                 & 80.5 & 76.7 & \textcolor{blue}{78.6} & 72.1 & 80.2 & \textcolor{red}{76.2} \\
\textbf{Qwen2.5-7B-Instruct}                & 81.7 & 79.4 & \textcolor{red}{80.6}  & 71.8 & 79.6 & 75.7 \\
\bottomrule
\end{tabular}
}
\end{table}


==> tables/knowledge_cleaning.tex <==
\begin{table}[t]
\centering
\small
\caption{Knowledge Extraction: Accuracy comparison on PubMedQA, Covert, and PubHealth under different reasoning and training settings.}
\label{tab:kbc-result}
\begin{tabular}{lccc}
\toprule
\textbf{Method (ACC)} & \textbf{PubMedQA} & \textbf{Covert} & \textbf{PubHealth} \\
\midrule
\textbf{CoT} & 36.40\% & 48.33\% & 29.00\% \\
\textbf{RAG} & 43.33\% & 17.55\% & 19.60\% \\
\textbf{SFT (DataFlow-Knowledge)} & \textbf{53.40\%} & \textbf{68.33\%} & \textbf{40.86\%} \\
\bottomrule
\end{tabular}

\end{table}


==> tables/reasoning.tex <==
\begin{table}[t]
\centering
\small
\caption{Math Reasoning Pipeline: Performance comparison of Qwen2.5-32B-Instruct under different synthetic data training settings.}
\resizebox{\textwidth}{!}{
\begin{tabular}{lccccccccc}
\toprule
\textbf{Model} & \textbf{gsm8k} & \textbf{math} & \textbf{amc23} & \textbf{olympiad} & \textbf{gaokao24\_mix} & \textbf{minerva} & \textbf{AIME24@32} & \textbf{AIME25@32} & \textbf{Avg} \\
\midrule
\textbf{Qwen2.5-32B-Instruct} & 95.8 & 73.5 & 70.0 & 38.5 & 42.9 & 26.5 & 16.8 & 11.6 & 46.95 \\
\midrule
\rowcolor[rgb]{.867, .922, .969}
\multicolumn{10}{c}{\textit{\textbf{Trained with 1 epoch}}} \\
\midrule
\textbf{+ SYNTHETIC-1-10k} & 92.9 & 71.8 & 52.5 & 38.4 & 23.1 & 24.3 & 35.6 & 34.0 & 46.6 \\
\textbf{+ Open-R1-10k}     & 91.5 & 72.3 & 65.0 & 38.4 & 20.9 & 24.6 & 43.0 & 33.5 & 48.7 \\
\textbf{+ DataFlow-Reasoning-10K} & 93.9 & 72.3 & 72.5 & 38.7 & 38.5 & 26.5 & 35.9 & 34.5 & \textbf{51.6} \\
\midrule
\rowcolor[rgb]{.867, .922, .969}
\multicolumn{10}{c}{\textit{\textbf{Trained with 2 epochs}}} \\
\midrule
\textbf{+ SYNTHETIC-1-10k}  & 94.5 & 78.4 & 75.0 & 45.0 & 24.2 & 28.3 & 48.4 & 37.9 & 54.0 \\
\textbf{+ Open-R1-10k}      & 93.9 & 77.2 & 80.0 & 44.1 & 20.9 & 25.4 & 51.0 & 40.7 & 54.2 \\
\textbf{+ DataFlow-Reasoning-10K} & 94.4 & 76.6 & 75.0 & 45.2 & 42.9 & 25.7 & 45.4 & 40.0 & \textbf{55.7} \\
\bottomrule
\end{tabular}
}
\label{tab:reasoning}
\end{table}


==> tables/text2sql.tex <==
\begin{table*}[t]
\centering
\caption{Text-to-SQL Pipeline: Performance of LLMs on mainstream benchmarks. The first two blocks list closed-source and open-source base models. The last two blocks show fine-tuned models, where the first column indicates the training data setting.}
\label{tab:text2sql_table}
\resizebox{\textwidth}{!}{
\begin{tabular}{l|cccccccccccccc|cc}
\toprule
\multirow{3}{*}{\textbf{LLM / Training Data}} & \multicolumn{2}{c}{\textbf{Spider}} & \multicolumn{2}{c}{\textbf{Spider}} & \multicolumn{2}{c}{\textbf{BIRD}} & \multicolumn{2}{c}{\multirow{2}{*}{\textbf{EHRSQL}}} & \multicolumn{2}{c}{\textbf{Spider-}} & \multicolumn{2}{c}{\textbf{Spider-}} & \multicolumn{2}{c|}{\textbf{Spider-}} & \multicolumn{2}{c}{\multirow{2}{*}{\textbf{Average}}}\\

& \multicolumn{2}{c}{\textbf{dev}} & \multicolumn{2}{c}{\textbf{test}} & \multicolumn{2}{c}{\textbf{dev}} & & & \multicolumn{2}{c}{\textbf{DK}}& \multicolumn{2}{c}{\textbf{Syn}} & \multicolumn{2}{c|}{\textbf{Realistic}} & &\\

\cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}
\cmidrule(lr){8-9}\cmidrule(lr){10-11}\cmidrule(lr){12-13}\cmidrule(lr){14-15}\cmidrule(lr){16-17}
& Gre & Maj & Gre & Maj & Gre & Maj & Gre & Maj & Gre & Maj & Gre & Maj & Gre & Maj &Gre & Maj\\

\midrule
\rowcolor[rgb]{.867, .922, .969}
\multicolumn{17}{c}{\textit{\textbf{Closed-source LLMs}}} \\
\midrule
GPT-4o-mini & 70.4 & 71.0 & 82.4 & 83.7 & 58.8 & 61.5 & 37.9 & 43.1 & 73.3 & 74.4 & 60.5 & 61.6 & 64.4 & 66.7 & 64.0 & 66.0 \\
GPT-4-Turbo & 72.4 & 72.2 & 83.4 & 84.2 & 62.0 & 63.6 & 43.1 & 44.8 & 72.3 & 72.1 & 62.9 & 63.5 & 67.5 & 68.3 & 66.2 & 67.0\\
GPT-4o & 70.9 & 70.7 & 83.2 & 84.9 & 61.9 & 64.0 & 44.9 & 45.5 & 72.9 & 73.5 & 59.6 & 62.3 & 66.5 & 66.7 & 65.7 & 66.8 \\
\midrule
\rowcolor[rgb]{.867, .922, .969}
\multicolumn{17}{c}{\textit{\textbf{Open-source LLMs}}} \\
\midrule
DeepSeek-Coder-7B-Instruct & 63.2 & 63.2 & 70.5 & 73.2 & 43.1 & 48.0 & 28.6 & 33.9 & 60.9 & 64.1 & 49.9 & 51.7 & 58.7 & 58.9 & 53.6 & 56.1 \\
Qwen2.5-Coder-7B-Instruct & 73.4 & 77.1 & 82.2 & 85.6 & 50.9 & 61.3 & 24.3 & 36.9 & 67.5 & 73.6 & 63.1 & 66.9 & 66.7 & 70.5 & 61.2 & 67.4\\
Qwen2.5-7B-Instruct & 65.4 & 68.9 & 76.8 & 82.6 & 46.9 & 56.4 & 20.9 & 32.1 & 63.7 & 71.8 & 54.2 & 60.0 & 56.7 & 63.6 & 54.9 & 62.2 \\
OpenCoder-8B-Instruct & 59.5 & 59.5 & 68.3 & 70.1 & 37.5 & 45.3 & 21.9 & 29.9 & 62.6 & 64.7 & 46.0 & 46.1 & 49.0 & 49.4 & 49.3 & 52.1 \\
Meta-Llama-3.1-8B-Instruct & 61.8 & 67.7 & 72.2 & 78.5 & 42.0 & 53.1 & 24.6 & 33.7 & 62.6 & 69.9 & 53.1 & 59.3 & 57.5 & 61.0 & 53.4 & 60.5 \\
Granite-8B-Code-Instruct & 58.5 & 59.2 & 64.9 & 68.6 & 27.6 & 32.5 & 16.0 & 22.6 & 50.7 & 54.4 & 45.0 & 46.8 & 48.8 & 49.4 & 44.5 & 47.6 \\
Granite-3.1-8B-Instruct & 58.3 & 65.0 & 69.8 & 75.3 & 36.0 & 47.2 & 19.6 & 32.3 & 60.0 & 66.5 & 47.7 & 53.8 & 46.5 & 57.1 & 48.3 & 56.7\\
\midrule
\rowcolor[rgb]{.867, .922, .969}
\multicolumn{17}{c}{\textit{\textbf{Trained on Meta-Llama-3.1-8B-Instruct}}} \\
\midrule
SynSQL(50K) & 67.1 & 73.9 & 72.7 & 78.6 & 49.1 & 55.2 & 33.6 & 40.8 & 63.8 & 66.1 & 59.6 & 63.5 & 69.3 & 71.6 & 59.3 & 64.2 \\

SynSQL(90K) & 68.2 & 74.6 & 73.4 & 78.5 & 51.1 & 54.9 & 31.8 & 38.0 & 61.8 & 67.4 & 58.9 & 63.6 & 69.0 & 70.9 & 59.2 & 64.0 \\

SynSQL(2.5M) & 70.6 & 73.7 & 78.3 & 82.5 & 58.9 & 62.0 & 35.1 & 37.0 & 72.3 & 74.7 & 61.0 & 63.1 & 67.9 & 69.4 & 63.4 & 66.1 \\
\midrule
Spider+BIRD+DataFlow-Text2SQL-90K & 74.9 & 79.2 & 78.4 & 82.3 & 53.4 & 58.9 & 28.4 & 36.5 & 67.7 & 69.7 & 66.6 & 69.1 & 74.4 & 75.0 & 63.4 & 67.2 \\
\midrule
\textbf{DataFlow-Text2SQL-50K} & 69.9 & 76.8 & 75.1 & 80.1 & 51.4 & 57.6 & 28.0 & 36.4 & 65.9 & 68.1 & 61.3 & 67.5 & 69.6 & 73.5 & 60.2 & 65.7 \\
\textbf{DataFlow-Text2SQL-90K} & 71.4 & 76.4 & 75.8 & 80.0 & 54.6 & 56.8 & 55.5 & 56.3 & 66.5 & 67.7 & 61.6 & 67.3 & 71.4 & 72.7 & 65.3 & 68.2 \\


\midrule
\rowcolor[rgb]{.867, .922, .969}
\multicolumn{17}{c}{\textit{\textbf{Trained on Qwen2.5-Coder-7B-Instruct}}} \\
\midrule
SynSQL(50K) & 77.1 & 82.1 & 81.8 & 84.8 & 54.0 & 59.3 & 33.1 & 44.1 & 67.1 & 69.5 & 68.0 & 70.6 & 77.2 & 80.3 & 65.5 & 70.1\\
SynSQL(90K) & 79.2 & 83.1 & 82.3 & 84.4 & 56.2 & 59.4 & 31.4 & 41.4 & 65.0 & 70.7 & 67.2 & 70.7 & 77.0 & 79.9 & 65.5 & 69.9 \\
SynSQL(2.5M) & 81.2 & 81.6 & 87.9 & 88.3 & 63.9 & 66.1 & 34.9 & 40.0 & 76.1 & 77.8 & 69.7 & 69.6 & 76.2 & 78.0 & 70.0 & 71.6 \\
\midrule
Spider+BIRD+DataFlow-Text2SQL-90K & 85.5 & 87.5 & 87.5 & 88.5 & 58.3 & 64.0 & 27.9 & 39.8 & 71.0 & 73.1 & 75.0 & 76.2 & 82.3 & 83.7 & 69.6 & 73.3 \\
\midrule
\textbf{DataFlow-Text2SQL-50K} & 80.9 & 84.9 & 84.6 & 85.8 & 57.9 & 62.5 & 27.8 & 39.4 & 69.7 & 71.2 & 70.0 & 74.0 & 77.8 & 82.1 & 67.0 & 71.4 \\
\textbf{DataFlow-Text2SQL-90K} & 82.0 & 85.0 & 84.8 & 86.0 & 59.2 & 61.5 & 56.1 & 58.7 & 69.7 & 71.0 & 69.9 & 74.4 & 79.5 & 81.7 & 71.6 & 74.0 \\
\bottomrule
\end{tabular}%
}
\end{table*}

==> tables/text_conversation.tex <==
\begin{table}[t]
\centering
\small
\caption{Conversation Synthesis: Performance comparison on conversation-domain datasets and general benchmarks for Qwen2.5-7B under different 15K SFT data sources.}
\label{tab:conversation}
% \resizebox{\textwidth}{!}{
\begin{tabular}{lcccccccc}
\toprule
& \multicolumn{3}{c}{\textbf{Conversation Benchmarks}} 
& \multicolumn{4}{c}{\textbf{General Benchmarks}} \\
\cmidrule(lr){2-4} \cmidrule(lr){5-8}
\textbf{Model} 
& \textbf{TopDial} & \textbf{Light} & \textbf{Avg} 
& \textbf{MMLU} & \textbf{AlpacaEval} & \textbf{Arena-Hard} & \textbf{Avg} \\
\midrule
\textbf{Qwen2.5-7B} 
& 7.71 & 7.79 & 7.75 
& 71.45 & 7.05 & 0.60 & 26.36 \\
\textbf{+ ShareGPT-15K} 
& 7.75 & 6.72 & 7.24 
& 73.09 & 3.70 & 1.30 & 26.03 \\
\textbf{+ UltraChat-15K} 
& 7.72 & 6.83 & 7.28 
& 72.97 & 3.97 & 0.80 & 25.91 \\
\textbf{+ DataFlow-Chat-15K} 
& 7.98 & 8.10 & 8.04 
& 73.41 & 10.11 & 1.10 & \textbf{28.21} \\
\bottomrule
\end{tabular}
% }
\end{table}


==> tables/text_pt.tex <==
\begin{table}[t]
\centering
\small
\caption{Pre-training Data Filtering: Performance comparison across models trained with 30B-scale tokens on general evaluation benchmarks.}
% \resizebox{\textwidth}{!}{
\label{tab:PT}
\begin{tabular}{lccccccc}
\toprule
\textbf{Methods} & \textbf{ARC-C} & \textbf{ARC-E} & \textbf{MMLU} & \textbf{HellaSwag} & \textbf{WinoGrande} & \textbf{Gaokao-MathQA} & \textbf{Avg} \\
\midrule
\textbf{Random-30B}      & 25.26 & 43.94 & 27.03 & 37.02 & 50.99 & 27.35 & 35.26 \\
\textbf{Qurating-30B}    & 25.00 & 43.14 & 27.50 & 37.03 & 50.67 & 26.78 & 35.02 \\
\textbf{FineWeb-Edu-30B}  & 26.45 & 45.41 & 27.41 & 38.06 & 50.43 & 25.64 & 35.57 \\
\textbf{DataFlow-30B}    & 25.51 & 45.58 & 27.42 & 37.58 & 50.67 & 27.35 & \textbf{35.69} \\
\bottomrule
\end{tabular}
% }
\end{table}


==> tables/text_sft.tex <==
\begin{table}[t]
\centering
\small
\caption{SFT Data Filtering: Comparison of different 5k dataset filtering methods across Math, Code, and Knowledge benchmarks.}
\label{tab:SFT}
\resizebox{\textwidth}{!}{
\begin{tabular}{lcccccccccccc}
\toprule
& \multicolumn{6}{c}{\textbf{Math}} & \multicolumn{3}{c}{\textbf{Code}} & \multicolumn{3}{c}{\textbf{Knowledge}} \\
\cmidrule(lr){2-7} \cmidrule(lr){8-10} \cmidrule(lr){11-13}
\textbf{Methods} & \textbf{math} & \textbf{gsm8k} & \textbf{aime24} & \textbf{minerva} & \textbf{olympiad} & \textbf{Avg} 
& \textbf{HumanEval} & \textbf{MBPP} & \textbf{Avg} 
& \textbf{MMLU} & \textbf{C-EVAL} & \textbf{Avg} \\
\midrule
\textbf{Alpaca(random)} 
& 54.9 & 77.2 & 13.3 & 14.0 & 27.0 & 37.3 
& 71.3 & 75.9 & 73.6 
& 71.8 & 80.0 & 75.9 \\
\textbf{Alpaca(filtered)} 
& 60.3 & 80.0 & 13.3 & 14.7 & 30.7 & 39.8 
& 73.8 & 75.7 & 74.8 
& 71.8 & 80.0 & 75.9 \\
\midrule
\textbf{WizardLM(random)} 
& 61.1 & 84.2 & 6.7 & 18.0 & 29.3 & 39.9 
& 75.6 & 82.0 & \textbf{78.8} 
& 71.8 & 79.2 & 75.5 \\
\textbf{WizardLM(filtered)} 
& 69.7 & 88.8 & 10.0 & 19.9 & 35.4 & 44.8 
& 77.4 & 80.4 & \textbf{78.9} 
& 71.9 & 79.6 & 75.8 \\
\midrule
\textbf{DataFlow-SFT-15K(random)} 
& 72.6 & 89.6 & 13.3 & 37.9 & 32.9 & \textbf{49.3} 
& 79.9 & 75.9 & 77.9 
& 72.1 & 80.0 & \textbf{76.1} \\
\textbf{DataFlow-SFT-15K(filtered)} 
& 73.3 & 90.2 & 13.3 & 36.0 & 35.9 & \textbf{49.7} 
& 82.9 & 74.9 & \textbf{78.9} 
& 72.2 & 80.4 & \textbf{76.3} \\
\bottomrule
\end{tabular}
}
\end{table}

